Near-Codewords Aware Bit Flipping Decoding of QC-MDPC Codes

Bit-Flipping (BF) decoders are a family of decoders widely employed in post-quantum cryptographic schemes based on Quasi-Cyclic Moderate-Density Parity-Check (QC-MDPC) codes, such as BIKE. BF decoders suffer from trapping sets, corresponding to low-weight error patterns that likely lead to decoding failures. For QC-MDPC codes, the most relevant family of trapping sets is that of near-codewords, which are error patterns associated to low-weight syndromes. Indeed, recent works show that error patterns having a large overlap with near-codewords are the main culprits for decoding failures at very low Decoding Failure Rate (DFR) values. In this paper, we show that any BF decoder can be tweaked and made somehow aware of near-codewords, which means being able to recognize, and recover from, bad configurations due to near-codewords. We show that this modification results in minimal computational overhead. Through intensive numerical simulations, we evaluate the effectiveness of this approach on several BF decoders, considering both toy code parameters and BIKE parameters for NIST security category 1. Our results show drastic reductions in the DFR. We also find that, with this modification, a recently proposed BF variant called BF-Max outperforms the two decoders used by BIKE within the NIST competition.

==> Data/mld_2003_11.tex <==
X Y Z
250 1.000000e+00 1.000000e+00
249 1.000000e+00 1.000000e+00
248 1.000000e+00 1.000000e+00
247 1.000000e+00 1.000000e+00
246 1.000000e+00 1.000000e+00
245 1.000000e+00 1.000000e+00
244 1.000000e+00 1.000000e+00
243 1.000000e+00 1.000000e+00
242 1.000000e+00 1.000000e+00
241 1.000000e+00 1.000000e+00
240 1.000000e+00 1.000000e+00
239 1.000000e+00 1.000000e+00
238 1.000000e+00 1.000000e+00
237 1.000000e+00 1.000000e+00
236 1.000000e+00 1.000000e+00
235 1.000000e+00 1.000000e+00
234 1.000000e+00 1.000000e+00
233 1.000000e+00 1.000000e+00
232 1.000000e+00 1.000000e+00
231 1.000000e+00 1.000000e+00
230 1.000000e+00 1.000000e+00
229 1.000000e+00 1.000000e+00
228 1.000000e+00 1.000000e+00
227 1.000000e+00 1.000000e+00
226 1.000000e+00 1.000000e+00
225 1.000000e+00 1.000000e+00
224 1.000000e+00 1.000000e+00
223 1.000000e+00 1.000000e+00
222 1.000000e+00 1.000000e+00
221 1.000000e+00 1.000000e+00
220 1.000000e+00 1.000000e+00
219 1.000000e+00 1.000000e+00
218 1.000000e+00 1.000000e+00
217 1.000000e+00 1.000000e+00
216 1.000000e+00 1.000000e+00
215 1.000000e+00 1.000000e+00
214 1.000000e+00 1.000000e+00
213 1.000000e+00 1.000000e+00
212 1.000000e+00 1.000000e+00
211 1.000000e+00 1.000000e+00
210 1.000000e+00 1.000000e+00
209 1.000000e+00 1.000000e+00
208 1.000000e+00 1.000000e+00
207 1.000000e+00 1.000000e+00
206 1.000000e+00 1.000000e+00
205 1.000000e+00 1.000000e+00
204 1.000000e+00 1.000000e+00
203 1.000000e+00 1.000000e+00
202 1.000000e+00 1.000000e+00
201 1.000000e+00 1.000000e+00
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 1.000000e+00 1.000000e+00
137 1.000000e+00 1.000000e+00
136 1.000000e+00 1.000000e+00
135 1.000000e+00 1.000000e+00
134 1.000000e+00 1.000000e+00
133 1.000000e+00 1.000000e+00
132 1.000000e+00 1.000000e+00
131 1.000000e+00 1.000000e+00
130 1.000000e+00 1.000000e+00
129 1.000000e+00 1.000000e+00
128 1.000000e+00 1.000000e+00
127 1.000000e+00 1.000000e+00
126 1.000000e+00 1.000000e+00
125 1.000000e+00 1.000000e+00
124 1.000000e+00 1.000000e+00
123 1.000000e+00 1.000000e+00
122 1.000000e+00 1.000000e+00
121 1.000000e+00 1.000000e+00
120 1.000000e+00 1.000000e+00
119 1.000000e+00 1.000000e+00
118 1.000000e+00 1.000000e+00
117 1.000000e+00 1.000000e+00
116 1.000000e+00 1.000000e+00
115 1.000000e+00 1.000000e+00
114 1.000000e+00 1.000000e+00
113 1.000000e+00 1.000000e+00
112 1.000000e+00 1.000000e+00
111 1.000000e+00 1.000000e+00
110 1.000000e+00 1.000000e+00
109 1.000000e+00 1.000000e+00
108 1.000000e+00 1.000000e+00
107 1.000000e+00 1.000000e+00
106 1.000000e+00 1.000000e+00
105 1.000000e+00 1.000000e+00
104 1.000000e+00 1.000000e+00
103 1.000000e+00 1.000000e+00
102 1.000000e+00 1.000000e+00
101 1.000000e+00 1.000000e+00
100 1.000000e+00 1.000000e+00
99 1.000000e+00 1.000000e+00
98 1.000000e+00 1.000000e+00
97 1.000000e+00 1.000000e+00
96 1.000000e+00 1.000000e+00
95 1.000000e+00 1.000000e+00
94 1.000000e+00 1.000000e+00
93 1.000000e+00 1.000000e+00
92 1.000000e+00 1.000000e+00
91 1.000000e+00 1.000000e+00
90 1.000000e+00 1.000000e+00
89 1.000000e+00 1.000000e+00
88 1.000000e+00 1.000000e+00
87 1.000000e+00 1.000000e+00
86 1.000000e+00 1.000000e+00
85 1.000000e+00 1.000000e+00
84 1.000000e+00 1.000000e+00
83 1.000000e+00 1.000000e+00
82 1.000000e+00 1.000000e+00
81 1.000000e+00 1.000000e+00
80 1.000000e+00 1.000000e+00
79 1.000000e+00 1.000000e+00
78 1.000000e+00 1.000000e+00
77 1.000000e+00 1.000000e+00
76 1.000000e+00 1.000000e+00
75 1.000000e+00 1.000000e+00
74 1.000000e+00 1.000000e+00
73 1.000000e+00 1.000000e+00
72 1.000000e+00 1.000000e+00
71 1.000000e+00 1.000000e+00
70 1.000000e+00 1.000000e+00
69 1.000000e+00 1.000000e+00
68 1.000000e+00 1.000000e+00
67 1.000000e+00 1.000000e+00
66 1.000000e+00 1.000000e+00
65 1.000000e+00 1.000000e+00
64 1.000000e+00 1.000000e+00
63 1.000000e+00 1.000000e+00
62 1.000000e+00 1.000000e+00
61 1.000000e+00 1.000000e+00
60 1.000000e+00 1.000000e+00
59 1.000000e+00 1.000000e+00
58 1.000000e+00 9.777778e-01
57 1.000000e+00 1.000000e+00
56 9.777778e-01 9.777778e-01
55 9.777778e-01 9.777778e-01
54 8.823529e-01 8.627451e-01
53 8.979592e-01 8.571429e-01
52 7.377049e-01 7.213115e-01
51 4.205607e-01 3.925234e-01
50 3.259259e-01 3.185185e-01
49 2.107623e-01 1.928251e-01
48 9.750000e-02 9.500000e-02
47 5.052879e-02 4.347826e-02
46 2.443730e-02 2.057878e-02
45 1.080066e-02 7.043907e-03
44 4.857264e-03 2.641670e-03
43 2.411325e-03 1.166770e-03
42 1.456322e-03 6.721484e-04
41 1.055432e-03 4.459574e-04
40 5.580190e-04 2.989388e-04
39 4.316177e-04 2.490102e-04
38 2.833401e-04 1.545492e-04
37 1.950671e-04 1.170403e-04
36 1.530430e-04 8.347803e-05
35 1.014556e-04 5.967976e-05
34 6.654151e-05 4.247330e-05
33 5.849905e-05 3.988572e-05
32 4.512984e-05 3.008656e-05
31 2.850024e-05 1.819164e-05
30 1.776208e-05 1.366314e-05
29 1.660565e-05 1.509605e-05
28 1.066263e-05 8.417863e-06
27 6.516833e-06 5.012948e-06
26 4.033016e-06 3.902918e-06
25 4.256910e-06 3.990854e-06
24 1.640157e-06 1.491051e-06
23 1.601343e-06 1.601343e-06
22 9.140250e-07 8.064926e-07
21 8.663803e-07 8.384326e-07
20 4.166145e-07 4.031753e-07
19 3.118546e-07 3.118546e-07
18 1.824418e-07 1.710392e-07
17 8.861285e-08 8.861285e-08
16 6.416749e-08 6.209757e-08
15 4.138172e-08 4.138172e-08
14 2.000000e-08 2.000000e-08
13 1.500000e-08 1.400000e-08
12 3.000000e-09 3.000000e-09
11 2.000000e-09 2.000000e-09

==> Data/mld_2003_13.tex <==
X Y Z
250 1.000000e+00 1.000000e+00
249 1.000000e+00 1.000000e+00
248 1.000000e+00 1.000000e+00
247 1.000000e+00 1.000000e+00
246 1.000000e+00 1.000000e+00
245 1.000000e+00 1.000000e+00
244 1.000000e+00 1.000000e+00
243 1.000000e+00 1.000000e+00
242 1.000000e+00 1.000000e+00
241 1.000000e+00 1.000000e+00
240 1.000000e+00 1.000000e+00
239 1.000000e+00 1.000000e+00
238 1.000000e+00 1.000000e+00
237 1.000000e+00 1.000000e+00
236 1.000000e+00 1.000000e+00
235 1.000000e+00 1.000000e+00
234 1.000000e+00 1.000000e+00
233 1.000000e+00 1.000000e+00
232 1.000000e+00 1.000000e+00
231 1.000000e+00 1.000000e+00
230 1.000000e+00 1.000000e+00
229 1.000000e+00 1.000000e+00
228 1.000000e+00 1.000000e+00
227 1.000000e+00 1.000000e+00
226 1.000000e+00 1.000000e+00
225 1.000000e+00 1.000000e+00
224 1.000000e+00 1.000000e+00
223 1.000000e+00 1.000000e+00
222 1.000000e+00 1.000000e+00
221 1.000000e+00 1.000000e+00
220 1.000000e+00 1.000000e+00
219 1.000000e+00 1.000000e+00
218 1.000000e+00 1.000000e+00
217 1.000000e+00 1.000000e+00
216 1.000000e+00 1.000000e+00
215 1.000000e+00 1.000000e+00
214 1.000000e+00 1.000000e+00
213 1.000000e+00 1.000000e+00
212 1.000000e+00 1.000000e+00
211 1.000000e+00 1.000000e+00
210 1.000000e+00 1.000000e+00
209 1.000000e+00 1.000000e+00
208 1.000000e+00 1.000000e+00
207 1.000000e+00 1.000000e+00
206 1.000000e+00 1.000000e+00
205 1.000000e+00 1.000000e+00
204 1.000000e+00 1.000000e+00
203 1.000000e+00 1.000000e+00
202 1.000000e+00 1.000000e+00
201 1.000000e+00 1.000000e+00
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 1.000000e+00 1.000000e+00
137 1.000000e+00 1.000000e+00
136 1.000000e+00 1.000000e+00
135 1.000000e+00 1.000000e+00
134 1.000000e+00 1.000000e+00
133 1.000000e+00 1.000000e+00
132 1.000000e+00 1.000000e+00
131 1.000000e+00 1.000000e+00
130 1.000000e+00 1.000000e+00
129 1.000000e+00 1.000000e+00
128 1.000000e+00 1.000000e+00
127 1.000000e+00 1.000000e+00
126 1.000000e+00 1.000000e+00
125 1.000000e+00 1.000000e+00
124 1.000000e+00 1.000000e+00
123 1.000000e+00 1.000000e+00
122 1.000000e+00 1.000000e+00
121 1.000000e+00 1.000000e+00
120 1.000000e+00 1.000000e+00
119 1.000000e+00 1.000000e+00
118 1.000000e+00 1.000000e+00
117 1.000000e+00 1.000000e+00
116 1.000000e+00 1.000000e+00
115 1.000000e+00 1.000000e+00
114 1.000000e+00 1.000000e+00
113 1.000000e+00 1.000000e+00
112 1.000000e+00 1.000000e+00
111 1.000000e+00 1.000000e+00
110 1.000000e+00 1.000000e+00
109 1.000000e+00 1.000000e+00
108 1.000000e+00 1.000000e+00
107 1.000000e+00 1.000000e+00
106 1.000000e+00 1.000000e+00
105 1.000000e+00 1.000000e+00
104 1.000000e+00 1.000000e+00
103 1.000000e+00 1.000000e+00
102 1.000000e+00 1.000000e+00
101 1.000000e+00 1.000000e+00
100 1.000000e+00 1.000000e+00
99 1.000000e+00 1.000000e+00
98 1.000000e+00 1.000000e+00
97 1.000000e+00 1.000000e+00
96 1.000000e+00 1.000000e+00
95 1.000000e+00 1.000000e+00
94 1.000000e+00 1.000000e+00
93 1.000000e+00 1.000000e+00
92 1.000000e+00 1.000000e+00
91 1.000000e+00 1.000000e+00
90 1.000000e+00 1.000000e+00
89 1.000000e+00 1.000000e+00
88 1.000000e+00 1.000000e+00
87 1.000000e+00 1.000000e+00
86 1.000000e+00 1.000000e+00
85 1.000000e+00 1.000000e+00
84 1.000000e+00 1.000000e+00
83 1.000000e+00 1.000000e+00
82 1.000000e+00 1.000000e+00
81 1.000000e+00 1.000000e+00
80 1.000000e+00 1.000000e+00
79 1.000000e+00 1.000000e+00
78 1.000000e+00 1.000000e+00
77 1.000000e+00 1.000000e+00
76 1.000000e+00 1.000000e+00
75 1.000000e+00 1.000000e+00
74 1.000000e+00 1.000000e+00
73 1.000000e+00 1.000000e+00
72 1.000000e+00 1.000000e+00
71 1.000000e+00 1.000000e+00
70 1.000000e+00 1.000000e+00
69 1.000000e+00 1.000000e+00
68 1.000000e+00 1.000000e+00
67 1.000000e+00 1.000000e+00
66 1.000000e+00 1.000000e+00
65 1.000000e+00 1.000000e+00
64 1.000000e+00 1.000000e+00
63 1.000000e+00 1.000000e+00
62 1.000000e+00 1.000000e+00
61 1.000000e+00 1.000000e+00
60 1.000000e+00 1.000000e+00
59 1.000000e+00 1.000000e+00
58 1.000000e+00 1.000000e+00
57 1.000000e+00 1.000000e+00
56 1.000000e+00 1.000000e+00
55 1.000000e+00 1.000000e+00
54 1.000000e+00 1.000000e+00
53 9.777778e-01 9.777778e-01
52 9.777778e-01 9.777778e-01
51 9.777778e-01 9.777778e-01
50 9.777778e-01 9.777778e-01
49 9.166667e-01 9.166667e-01
48 8.800000e-01 8.800000e-01
47 6.428571e-01 6.142857e-01
46 4.673913e-01 4.673913e-01
45 4.000000e-01 4.000000e-01
44 2.206573e-01 2.065728e-01
43 1.105121e-01 1.105121e-01
42 4.891923e-02 4.550626e-02
41 2.144608e-02 2.022059e-02
40 1.071975e-02 9.800918e-03
39 3.008424e-03 2.481950e-03
38 1.172826e-03 6.859925e-04
37 4.077216e-04 1.568160e-04
36 2.168487e-04 4.748511e-05
35 1.080770e-04 1.232818e-05
34 6.089517e-05 6.455318e-06
33 3.580412e-05 3.388403e-06
32 2.177325e-05 2.815506e-06
31 1.559400e-05 1.933141e-06
30 8.457308e-06 1.098352e-06
29 5.643780e-06 8.958381e-07
28 3.452872e-06 4.795655e-07
27 1.926754e-06 2.438929e-07
26 1.321751e-06 2.509653e-07
25 7.155314e-07 1.866604e-07
24 4.068435e-07 1.173587e-07
23 2.460236e-07 5.197682e-08
22 1.345038e-07 3.033921e-08

==> Data/mld_2003_15.tex <==
X Y Z
250 1.000000e+00 1.000000e+00
249 1.000000e+00 1.000000e+00
248 1.000000e+00 1.000000e+00
247 1.000000e+00 1.000000e+00
246 1.000000e+00 1.000000e+00
245 1.000000e+00 1.000000e+00
244 1.000000e+00 1.000000e+00
243 1.000000e+00 1.000000e+00
242 1.000000e+00 1.000000e+00
241 1.000000e+00 1.000000e+00
240 1.000000e+00 1.000000e+00
239 1.000000e+00 1.000000e+00
238 1.000000e+00 1.000000e+00
237 1.000000e+00 1.000000e+00
236 1.000000e+00 1.000000e+00
235 1.000000e+00 1.000000e+00
234 1.000000e+00 1.000000e+00
233 1.000000e+00 1.000000e+00
232 1.000000e+00 1.000000e+00
231 1.000000e+00 1.000000e+00
230 1.000000e+00 1.000000e+00
229 1.000000e+00 1.000000e+00
228 1.000000e+00 1.000000e+00
227 1.000000e+00 1.000000e+00
226 1.000000e+00 1.000000e+00
225 1.000000e+00 1.000000e+00
224 1.000000e+00 1.000000e+00
223 1.000000e+00 1.000000e+00
222 1.000000e+00 1.000000e+00
221 1.000000e+00 1.000000e+00
220 1.000000e+00 1.000000e+00
219 1.000000e+00 1.000000e+00
218 1.000000e+00 1.000000e+00
217 1.000000e+00 1.000000e+00
216 1.000000e+00 1.000000e+00
215 1.000000e+00 1.000000e+00
214 1.000000e+00 1.000000e+00
213 1.000000e+00 1.000000e+00
212 1.000000e+00 1.000000e+00
211 1.000000e+00 1.000000e+00
210 1.000000e+00 1.000000e+00
209 1.000000e+00 1.000000e+00
208 1.000000e+00 1.000000e+00
207 1.000000e+00 1.000000e+00
206 1.000000e+00 1.000000e+00
205 1.000000e+00 1.000000e+00
204 1.000000e+00 1.000000e+00
203 1.000000e+00 1.000000e+00
202 1.000000e+00 1.000000e+00
201 1.000000e+00 1.000000e+00
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 1.000000e+00 1.000000e+00
137 1.000000e+00 1.000000e+00
136 1.000000e+00 1.000000e+00
135 1.000000e+00 1.000000e+00
134 1.000000e+00 1.000000e+00
133 1.000000e+00 1.000000e+00
132 1.000000e+00 1.000000e+00
131 1.000000e+00 1.000000e+00
130 1.000000e+00 1.000000e+00
129 1.000000e+00 1.000000e+00
128 1.000000e+00 1.000000e+00
127 1.000000e+00 1.000000e+00
126 1.000000e+00 1.000000e+00
125 1.000000e+00 1.000000e+00
124 1.000000e+00 1.000000e+00
123 1.000000e+00 1.000000e+00
122 1.000000e+00 1.000000e+00
121 1.000000e+00 1.000000e+00
120 1.000000e+00 1.000000e+00
119 1.000000e+00 1.000000e+00
118 1.000000e+00 1.000000e+00
117 1.000000e+00 1.000000e+00
116 1.000000e+00 1.000000e+00
115 1.000000e+00 1.000000e+00
114 1.000000e+00 1.000000e+00
113 1.000000e+00 1.000000e+00
112 1.000000e+00 1.000000e+00
111 1.000000e+00 1.000000e+00
110 1.000000e+00 1.000000e+00
109 1.000000e+00 1.000000e+00
108 1.000000e+00 1.000000e+00
107 1.000000e+00 1.000000e+00
106 1.000000e+00 1.000000e+00
105 1.000000e+00 1.000000e+00
104 1.000000e+00 1.000000e+00
103 1.000000e+00 1.000000e+00
102 1.000000e+00 1.000000e+00
101 1.000000e+00 1.000000e+00
100 1.000000e+00 1.000000e+00
99 1.000000e+00 1.000000e+00
98 1.000000e+00 1.000000e+00
97 1.000000e+00 1.000000e+00
96 1.000000e+00 1.000000e+00
95 1.000000e+00 1.000000e+00
94 1.000000e+00 1.000000e+00
93 1.000000e+00 1.000000e+00
92 1.000000e+00 1.000000e+00
91 1.000000e+00 1.000000e+00
90 1.000000e+00 1.000000e+00
89 1.000000e+00 1.000000e+00
88 1.000000e+00 1.000000e+00
87 1.000000e+00 1.000000e+00
86 1.000000e+00 1.000000e+00
85 1.000000e+00 1.000000e+00
84 1.000000e+00 1.000000e+00
83 1.000000e+00 1.000000e+00
82 1.000000e+00 1.000000e+00
81 1.000000e+00 1.000000e+00
80 1.000000e+00 1.000000e+00
79 1.000000e+00 1.000000e+00
78 1.000000e+00 1.000000e+00
77 1.000000e+00 1.000000e+00
76 1.000000e+00 1.000000e+00
75 1.000000e+00 1.000000e+00
74 1.000000e+00 1.000000e+00
73 1.000000e+00 1.000000e+00
72 1.000000e+00 1.000000e+00
71 1.000000e+00 1.000000e+00
70 1.000000e+00 1.000000e+00
69 1.000000e+00 1.000000e+00
68 1.000000e+00 1.000000e+00
67 1.000000e+00 1.000000e+00
66 1.000000e+00 1.000000e+00
65 1.000000e+00 1.000000e+00
64 1.000000e+00 1.000000e+00
63 1.000000e+00 1.000000e+00
62 1.000000e+00 1.000000e+00
61 1.000000e+00 1.000000e+00
60 1.000000e+00 1.000000e+00
59 1.000000e+00 1.000000e+00
58 1.000000e+00 1.000000e+00
57 1.000000e+00 1.000000e+00
56 1.000000e+00 1.000000e+00
55 1.000000e+00 1.000000e+00
54 1.000000e+00 1.000000e+00
53 1.000000e+00 1.000000e+00
52 1.000000e+00 1.000000e+00
51 1.000000e+00 1.000000e+00
50 1.000000e+00 1.000000e+00
49 1.000000e+00 1.000000e+00
48 9.777778e-01 9.777778e-01
47 9.361702e-01 9.361702e-01
46 9.166667e-01 9.166667e-01
45 8.000000e-01 8.000000e-01
44 6.984127e-01 6.984127e-01
43 4.313726e-01 4.313726e-01
42 3.153846e-01 3.153846e-01
41 1.578947e-01 1.578947e-01
40 7.847083e-02 7.847083e-02
39 2.389079e-02 2.252560e-02
38 6.128134e-03 6.128134e-03
37 1.335644e-03 1.119053e-03
36 3.128044e-04 2.681181e-04
35 3.552290e-05 2.599237e-05
34 1.173529e-05 3.418047e-06
33 4.933453e-06 7.668579e-07
32 2.392719e-06 4.125378e-07
31 1.363531e-06 2.420469e-07
30 8.324433e-07 2.134470e-07
29 4.239642e-07 8.049953e-08
28 2.098804e-07 5.077753e-08
27 1.220000e-07 2.800000e-08
26 7.097792e-08 2.681388e-08

==> Data/mld_2003_9.tex <==
X Y Z
250 1.000000e+00 1.000000e+00
249 1.000000e+00 1.000000e+00
248 1.000000e+00 1.000000e+00
247 1.000000e+00 1.000000e+00
246 1.000000e+00 1.000000e+00
245 1.000000e+00 1.000000e+00
244 1.000000e+00 1.000000e+00
243 1.000000e+00 1.000000e+00
242 1.000000e+00 1.000000e+00
241 1.000000e+00 1.000000e+00
240 1.000000e+00 1.000000e+00
239 1.000000e+00 1.000000e+00
238 1.000000e+00 1.000000e+00
237 1.000000e+00 1.000000e+00
236 1.000000e+00 1.000000e+00
235 1.000000e+00 1.000000e+00
234 1.000000e+00 1.000000e+00
233 1.000000e+00 1.000000e+00
232 1.000000e+00 1.000000e+00
231 1.000000e+00 1.000000e+00
230 1.000000e+00 1.000000e+00
229 1.000000e+00 1.000000e+00
228 1.000000e+00 1.000000e+00
227 1.000000e+00 1.000000e+00
226 1.000000e+00 1.000000e+00
225 1.000000e+00 1.000000e+00
224 1.000000e+00 1.000000e+00
223 1.000000e+00 1.000000e+00
222 1.000000e+00 1.000000e+00
221 1.000000e+00 1.000000e+00
220 1.000000e+00 1.000000e+00
219 1.000000e+00 1.000000e+00
218 1.000000e+00 1.000000e+00
217 1.000000e+00 1.000000e+00
216 1.000000e+00 1.000000e+00
215 1.000000e+00 1.000000e+00
214 1.000000e+00 1.000000e+00
213 1.000000e+00 1.000000e+00
212 1.000000e+00 1.000000e+00
211 1.000000e+00 1.000000e+00
210 1.000000e+00 1.000000e+00
209 1.000000e+00 1.000000e+00
208 1.000000e+00 1.000000e+00
207 1.000000e+00 1.000000e+00
206 1.000000e+00 1.000000e+00
205 1.000000e+00 1.000000e+00
204 1.000000e+00 1.000000e+00
203 1.000000e+00 1.000000e+00
202 1.000000e+00 1.000000e+00
201 1.000000e+00 1.000000e+00
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 9.600000e-01 9.600000e-01
141 9.583333e-01 9.583333e-01
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 9.583333e-01 9.583333e-01
137 8.846154e-01 8.846154e-01
136 8.461539e-01 8.076923e-01
135 9.200000e-01 9.200000e-01
134 7.692308e-01 7.692308e-01
133 9.200000e-01 9.200000e-01
132 6.785714e-01 6.785714e-01
131 7.333333e-01 7.333333e-01
130 5.789474e-01 5.000000e-01
129 5.526316e-01 4.473684e-01
128 5.161290e-01 5.161290e-01
127 4.615385e-01 4.358974e-01
126 3.400000e-01 2.800000e-01
125 3.571429e-01 3.095238e-01
124 2.388060e-01 1.940299e-01
123 1.827957e-01 1.075269e-01
122 2.089552e-01 1.791045e-01
121 1.652174e-01 1.130435e-01
120 1.272727e-01 6.666667e-02
119 9.952607e-02 5.213270e-02
118 1.013216e-01 4.405286e-02
117 6.910569e-02 4.065040e-02
116 5.726872e-02 1.468429e-02
115 4.470199e-02 1.655629e-02
114 3.968872e-02 7.782101e-03
113 3.861386e-02 9.900990e-03
112 2.333212e-02 3.645643e-03
111 2.781955e-02 3.759399e-03
110 2.076647e-02 1.887861e-03
109 2.184793e-02 9.624639e-04
108 1.752168e-02 9.031792e-04
107 1.607851e-02 5.220296e-04
106 1.388157e-02 5.857201e-04
105 1.285824e-02 3.198567e-04
104 1.139833e-02 6.784721e-04
103 1.144700e-02 1.966839e-04
102 9.985848e-03 1.322629e-04
101 8.631161e-03 1.065575e-04

==> Data/out_2003_11.tex <==
X Y Z
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 1.000000e+00 1.000000e+00
137 1.000000e+00 1.000000e+00
136 1.000000e+00 1.000000e+00
135 1.000000e+00 1.000000e+00
134 1.000000e+00 1.000000e+00
133 1.000000e+00 1.000000e+00
132 1.000000e+00 1.000000e+00
131 1.000000e+00 1.000000e+00
130 1.000000e+00 1.000000e+00
129 1.000000e+00 1.000000e+00
128 9.777778e-01 9.777778e-01
127 1.000000e+00 1.000000e+00
126 9.361702e-01 9.148936e-01
125 9.555556e-01 9.555556e-01
124 9.111111e-01 9.111111e-01
123 9.318182e-01 9.318182e-01
122 8.723404e-01 8.723404e-01
121 8.333333e-01 8.333333e-01
120 7.843137e-01 7.843137e-01
119 7.049180e-01 7.049180e-01
118 6.290323e-01 6.290323e-01
117 5.142857e-01 5.142857e-01
116 4.523810e-01 4.523810e-01
115 3.303571e-01 3.214286e-01
114 2.704918e-01 2.704918e-01
113 1.588785e-01 1.448598e-01
112 1.800000e-01 1.700000e-01
111 1.147541e-01 1.081967e-01
110 1.009174e-01 9.174312e-02
109 6.517691e-02 5.772812e-02
108 4.993065e-02 4.160888e-02
107 3.671329e-02 2.622378e-02
106 2.668035e-02 1.539251e-02
105 1.506932e-02 9.041592e-03
104 1.364860e-02 5.767012e-03
103 7.295466e-03 2.605524e-03
102 6.774170e-03 2.208968e-03
101 5.208695e-03 1.041739e-03
100 3.823983e-03 4.248871e-04
99 3.403853e-03 2.363787e-04
98 2.887213e-03 1.592213e-04
97 2.216940e-03 5.932934e-05
96 1.903291e-03 3.207794e-05
95 1.676773e-03 1.640143e-05
94 1.438517e-03 1.169526e-05
93 1.227844e-03 4.518561e-06
92 1.067640e-03 3.475391e-06
91 9.147843e-04 2.492374e-06
90 7.859187e-04 1.707405e-06
89 6.825155e-04 1.314046e-06
88 5.916593e-04 6.488915e-07
87 5.103124e-04 6.468111e-07
86 4.343826e-04 3.793735e-07
85 3.752927e-04 3.502716e-07
84 3.216253e-04 3.313561e-07
83 2.779025e-04 2.082030e-07
82 2.396143e-04 2.228210e-07
81 2.041807e-04 1.458538e-07
80 1.732212e-04 8.611116e-08
79 1.465119e-04 7.669039e-08
78 1.261304e-04 5.120177e-08

==> Data/out_2003_13.tex <==
X Y Z
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 1.000000e+00 1.000000e+00
137 1.000000e+00 1.000000e+00
136 1.000000e+00 1.000000e+00
135 1.000000e+00 1.000000e+00
134 1.000000e+00 1.000000e+00
133 1.000000e+00 1.000000e+00
132 1.000000e+00 1.000000e+00
131 1.000000e+00 1.000000e+00
130 1.000000e+00 1.000000e+00
129 1.000000e+00 1.000000e+00
128 1.000000e+00 1.000000e+00
127 1.000000e+00 1.000000e+00
126 1.000000e+00 1.000000e+00
125 1.000000e+00 1.000000e+00
124 1.000000e+00 1.000000e+00
123 1.000000e+00 1.000000e+00
122 1.000000e+00 1.000000e+00
121 1.000000e+00 1.000000e+00
120 1.000000e+00 1.000000e+00
119 1.000000e+00 1.000000e+00
118 1.000000e+00 1.000000e+00
117 9.767442e-01 9.767442e-01
116 1.000000e+00 1.000000e+00
115 9.756098e-01 9.756098e-01
114 1.000000e+00 1.000000e+00
113 9.318182e-01 9.318182e-01
112 9.555556e-01 9.555556e-01
111 8.863636e-01 8.863636e-01
110 8.750000e-01 8.750000e-01
109 8.297873e-01 8.297873e-01
108 7.735849e-01 7.735849e-01
107 5.781250e-01 5.781250e-01
106 6.607143e-01 6.428571e-01
105 5.211267e-01 5.211267e-01
104 5.000000e-01 4.868421e-01
103 2.661290e-01 2.661290e-01
102 2.500000e-01 2.500000e-01
101 1.606218e-01 1.606218e-01
100 1.845238e-01 1.845238e-01
99 8.908046e-02 8.620690e-02
98 7.172131e-02 6.762295e-02
97 5.691057e-02 5.365854e-02
96 2.171291e-02 1.809409e-02
95 1.823529e-02 1.764706e-02
94 9.318837e-03 6.878189e-03
93 4.479961e-03 3.632401e-03
92 2.827712e-03 2.019794e-03
91 1.867930e-03 1.037739e-03
90 1.211477e-03 6.376196e-04
89 9.020037e-04 3.221442e-04
88 6.576063e-04 1.603918e-04
87 4.409139e-04 7.307965e-05
86 3.681128e-04 4.822438e-05
85 2.963155e-04 4.233079e-05
84 2.335641e-04 1.898895e-05
83 1.989387e-04 1.830724e-05
82 1.789357e-04 1.597641e-05
81 1.243784e-04 1.337403e-05
80 1.195596e-04 8.226578e-06
79 9.050412e-05 9.362495e-06
78 8.603449e-05 6.341609e-06
77 7.402009e-05 5.116596e-06
76 5.724492e-05 5.349993e-06
75 4.880272e-05 5.786884e-06
74 4.399260e-05 4.011484e-06
73 3.479916e-05 3.728481e-06
72 3.018577e-05 2.687161e-06
71 2.565806e-05 2.412983e-06
70 2.025480e-05 2.430576e-06
69 1.831879e-05 1.650341e-06
68 1.310747e-05 1.638433e-06
67 1.289971e-05 1.639794e-06
66 1.134943e-05 1.238120e-06
65 9.498703e-06 1.417717e-06
64 7.886528e-06 8.961964e-07
63 6.709283e-06 8.083474e-07
62 6.583826e-06 1.056229e-06
61 4.729726e-06 6.391521e-07
60 4.015181e-06 5.763418e-07
59 3.207714e-06 5.038294e-07
58 2.860930e-06 4.904451e-07
57 2.478958e-06 5.059097e-07
56 2.064446e-06 3.499061e-07
55 1.663637e-06 2.198639e-07
54 1.446482e-06 2.169722e-07
53 1.198193e-06 1.728163e-07
52 1.159048e-06 1.783150e-07
51 8.606184e-07 1.373327e-07
50 7.938657e-07 1.208933e-07
49 6.992002e-07 1.098220e-07
48 5.468914e-07 8.868509e-08

==> Data/out_2003_15.tex <==
X Y Z
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 1.000000e+00 1.000000e+00
139 1.000000e+00 1.000000e+00
138 1.000000e+00 1.000000e+00
137 1.000000e+00 1.000000e+00
136 1.000000e+00 1.000000e+00
135 1.000000e+00 1.000000e+00
134 1.000000e+00 1.000000e+00
133 1.000000e+00 1.000000e+00
132 1.000000e+00 1.000000e+00
131 1.000000e+00 1.000000e+00
130 1.000000e+00 1.000000e+00
129 1.000000e+00 1.000000e+00
128 1.000000e+00 1.000000e+00
127 1.000000e+00 1.000000e+00
126 1.000000e+00 1.000000e+00
125 1.000000e+00 1.000000e+00
124 1.000000e+00 1.000000e+00
123 1.000000e+00 1.000000e+00
122 1.000000e+00 1.000000e+00
121 1.000000e+00 1.000000e+00
120 1.000000e+00 1.000000e+00
119 1.000000e+00 1.000000e+00
118 1.000000e+00 1.000000e+00
117 1.000000e+00 1.000000e+00
116 1.000000e+00 1.000000e+00
115 1.000000e+00 1.000000e+00
114 1.000000e+00 1.000000e+00
113 1.000000e+00 1.000000e+00
112 1.000000e+00 1.000000e+00
111 1.000000e+00 1.000000e+00
110 1.000000e+00 1.000000e+00
109 1.000000e+00 1.000000e+00
108 1.000000e+00 1.000000e+00
107 1.000000e+00 1.000000e+00
106 1.000000e+00 1.000000e+00
105 1.000000e+00 1.000000e+00
104 9.512195e-01 9.512195e-01
103 1.000000e+00 1.000000e+00
102 1.000000e+00 1.000000e+00
101 9.130435e-01 9.130435e-01
100 9.523810e-01 9.523810e-01
99 9.090909e-01 9.090909e-01
98 8.571429e-01 8.571429e-01
97 7.291667e-01 7.291667e-01
96 6.491228e-01 6.491228e-01
95 5.538462e-01 5.538462e-01
94 3.854167e-01 3.854167e-01
93 3.932584e-01 3.932584e-01
92 3.274336e-01 3.274336e-01
91 1.857924e-01 1.857924e-01
90 1.797753e-01 1.797753e-01
89 1.063123e-01 1.063123e-01
88 9.041096e-02 8.767124e-02
87 4.073587e-02 4.073587e-02
86 2.368220e-02 2.368220e-02
85 1.220008e-02 1.220008e-02
84 8.653014e-03 8.653014e-03
83 4.466215e-03 4.322144e-03
82 1.760977e-03 1.760977e-03
81 6.866717e-04 6.866717e-04
80 3.969270e-04 3.841229e-04
79 1.741601e-04 1.632751e-04
78 6.651308e-05 4.534983e-05
77 4.635197e-05 2.575109e-05
76 2.129687e-05 9.982906e-06
75 1.582535e-05 6.782294e-06
74 1.132916e-05 3.398747e-06
73 8.501957e-06 2.040470e-06
72 7.199612e-06 1.648766e-06
71 5.241978e-06 1.332706e-06
70 3.954446e-06 1.395687e-06
69 2.923336e-06 5.965992e-07
68 2.297197e-06 6.265083e-07
67 2.229656e-06 6.688968e-07
66 1.623736e-06 5.127586e-07
65 1.335014e-06 4.767907e-07
64 1.007247e-06 3.214617e-07
63 9.382548e-07 2.490942e-07
62 7.276300e-07 2.250402e-07
61 5.513753e-07 1.117653e-07
60 5.784314e-07 2.058824e-07
59 3.893986e-07 1.168196e-07
58 3.478803e-07 1.033308e-07

==> Data/out_2003_9.tex <==
X Y Z
200 1.000000e+00 1.000000e+00
199 1.000000e+00 1.000000e+00
198 1.000000e+00 1.000000e+00
197 1.000000e+00 1.000000e+00
196 1.000000e+00 1.000000e+00
195 1.000000e+00 1.000000e+00
194 1.000000e+00 1.000000e+00
193 1.000000e+00 1.000000e+00
192 1.000000e+00 1.000000e+00
191 1.000000e+00 1.000000e+00
190 1.000000e+00 1.000000e+00
189 1.000000e+00 1.000000e+00
188 1.000000e+00 1.000000e+00
187 1.000000e+00 1.000000e+00
186 1.000000e+00 1.000000e+00
185 1.000000e+00 1.000000e+00
184 1.000000e+00 1.000000e+00
183 1.000000e+00 1.000000e+00
182 1.000000e+00 1.000000e+00
181 1.000000e+00 1.000000e+00
180 1.000000e+00 1.000000e+00
179 1.000000e+00 1.000000e+00
178 1.000000e+00 1.000000e+00
177 1.000000e+00 1.000000e+00
176 1.000000e+00 1.000000e+00
175 1.000000e+00 1.000000e+00
174 1.000000e+00 1.000000e+00
173 1.000000e+00 1.000000e+00
172 1.000000e+00 1.000000e+00
171 1.000000e+00 1.000000e+00
170 1.000000e+00 1.000000e+00
169 1.000000e+00 1.000000e+00
168 1.000000e+00 1.000000e+00
167 1.000000e+00 1.000000e+00
166 1.000000e+00 1.000000e+00
165 1.000000e+00 1.000000e+00
164 1.000000e+00 1.000000e+00
163 1.000000e+00 1.000000e+00
162 1.000000e+00 1.000000e+00
161 1.000000e+00 1.000000e+00
160 1.000000e+00 1.000000e+00
159 1.000000e+00 1.000000e+00
158 1.000000e+00 1.000000e+00
157 1.000000e+00 1.000000e+00
156 1.000000e+00 1.000000e+00
155 1.000000e+00 1.000000e+00
154 1.000000e+00 1.000000e+00
153 1.000000e+00 1.000000e+00
152 1.000000e+00 1.000000e+00
151 1.000000e+00 1.000000e+00
150 1.000000e+00 1.000000e+00
149 1.000000e+00 1.000000e+00
148 1.000000e+00 1.000000e+00
147 1.000000e+00 1.000000e+00
146 1.000000e+00 1.000000e+00
145 1.000000e+00 1.000000e+00
144 1.000000e+00 1.000000e+00
143 1.000000e+00 1.000000e+00
142 1.000000e+00 1.000000e+00
141 1.000000e+00 1.000000e+00
140 9.772727e-01 9.772727e-01
139 1.000000e+00 1.000000e+00
138 9.130435e-01 9.130435e-01
137 9.767442e-01 9.767442e-01
136 8.979592e-01 8.979592e-01
135 8.627451e-01 8.235294e-01
134 8.163266e-01 8.163266e-01
133 8.235294e-01 7.843137e-01
132 8.076923e-01 7.884616e-01
131 6.093750e-01 5.781250e-01
130 5.522388e-01 5.373135e-01
129 4.823529e-01 4.588235e-01
128 5.125000e-01 4.750000e-01
127 3.846154e-01 3.173077e-01
126 3.714286e-01 3.238095e-01
125 4.404762e-01 4.047619e-01
124 2.580645e-01 2.064516e-01
123 2.056075e-01 1.542056e-01
122 2.100840e-01 1.386555e-01
121 1.660900e-01 1.141869e-01
120 1.033708e-01 6.741573e-02
119 1.051625e-01 6.118547e-02
118 8.343266e-02 3.575685e-02
117 9.129815e-02 4.564907e-02
116 4.521556e-02 1.577287e-02
115 4.485488e-02 1.130795e-02
114 4.579310e-02 8.275862e-03
113 2.917673e-02 5.575172e-03
112 3.050569e-02 3.519887e-03
111 2.682275e-02 2.765232e-03
110 2.473817e-02 2.708559e-03
109 2.291214e-02 1.277629e-03
108 1.660116e-02 7.757551e-04
107 1.752990e-02 8.230001e-04
106 1.543665e-02 4.974217e-04
105 1.346149e-02 3.774250e-04
104 1.211588e-02 2.467592e-04
103 1.145498e-02 2.257880e-04
102 1.029972e-02 1.696823e-04
101 9.019424e-03 1.208498e-04
100 7.893838e-03 8.068659e-05
99 7.435189e-03 8.582365e-05
98 6.557345e-03 7.205874e-05
97 5.913246e-03 4.478601e-05
96 5.530337e-03 5.290502e-05
95 4.661214e-03 4.242609e-05
94 4.346380e-03 3.752270e-05
93 3.848901e-03 2.494427e-05
92 3.492940e-03 1.846488e-05
91 3.150875e-03 1.563451e-05
90 2.863651e-03 1.238603e-05
89 2.495207e-03 1.107177e-05
88 2.192591e-03 1.202298e-05
87 1.986489e-03 9.034971e-06
86 1.773852e-03 6.350307e-06
85 1.551735e-03 7.418655e-06
84 1.380519e-03 3.570923e-06
83 1.243883e-03 3.931777e-06
82 1.086424e-03 3.018962e-06
81 9.532723e-04 3.023382e-06
80 8.384524e-04 2.113568e-06
79 7.221632e-04 1.657732e-06
78 6.256969e-04 1.518805e-06
77 5.595234e-04 1.517557e-06
76 4.918398e-04 1.071080e-06
75 4.219331e-04 6.296257e-07
74 3.670985e-04 7.217824e-07
73 3.199928e-04 4.240562e-07
72 2.773767e-04 4.362640e-07
71 2.375357e-04 3.986837e-07
70 1.997113e-04 3.729204e-07
69 1.711810e-04 2.967427e-07
68 1.482293e-04 1.871740e-07
67 1.255333e-04 2.070596e-07
66 1.072829e-04 1.987087e-07
65 9.099219e-05 1.068862e-07
64 7.688577e-05 7.033951e-08
63 6.470711e-05 5.885317e-08
62 5.450619e-05 7.887255e-08
